SALAD: Part-Level Latent Diffusion for 3D Shape Generation and Manipulation

We present a cascaded diffusion model based on a part-level implicit 3D representation. Our model achieves state-of-the-art generation quality and also enables part-level shape editing and manipulation without any additional training in conditional setup. Diffusion models have demonstrated impressive capabilities in data generation as well as zero-shot completion and editing via a guided reverse process. Recent research on 3D diffusion models has focused on improving their generation capabilities with various data representations, while the absence of structural information has limited their capability in completion and editing tasks. We thus propose our novel diffusion model using a part-level implicit representation. To effectively learn diffusion with high-dimensional embedding vectors of parts, we propose a cascaded framework, learning diffusion first on a low-dimensional subspace encoding extrinsic parameters of parts and then on the other high-dimensional subspace encoding intrinsic attributes. In the experiments, we demonstrate the outperformance of our method compared with the previous ones both in generation and part-level completion and manipulation tasks.

==> figures/ablation_comparison.tex <==
\setlength{\tabcolsep}{0em}
\def\arraystretch{0.0}
%\newcolumntype{Y}{>{\centering\arraybackslash}m{0.0909\textwidth}}
\begin{figure*}
{\scriptsize
\begin{tabularx}{\linewidth}{YYYY}
SPAGHETTI & $\B{z}$ & $\{\B{e}_i\}_{i=1}^N\}, \{\B{s}_i\}_{i=1}^N\}$ & Ours \\  
\midrule
\multicolumn{4}{c}{\includegraphics[width=\linewidth]{figures/fig_ablation_chair.png}} \\
\multicolumn{7}{c}{\includegraphics[width=\linewidth]{figures/fig_ablation_airplane.png}} 
\end{tabularx}
}
\caption{Ablation studies.}
\label{fig:ablation_study}
\vspace{-0.5\baselineskip}
\end{figure*}

==> figures/part_completion/airplane_list.tex <==
\Image{figures/part_completion/airplanes/3.png}
\Image{figures/part_completion/airplanes/4.png}
\Image{figures/part_completion/airplanes/18.png}
\Image{figures/part_completion/airplanes/25.png}
\Image{figures/part_completion/airplanes/29.png}
\Image{figures/part_completion/airplanes/30.png}
\Image{figures/part_completion/airplanes/32.png}
\Image{figures/part_completion/airplanes/39.png}
\Image{figures/part_completion/airplanes/55.png}
\Image{figures/part_completion/airplanes/59.png}
\Image{figures/part_completion/airplanes/65.png}
\Image{figures/part_completion/airplanes/76.png}
\Image{figures/part_completion/airplanes/75.png}
\Image{figures/part_completion/airplanes/77.png}
\Image{figures/part_completion/airplanes/180.png}

==> figures/part_completion/chair_list.tex <==
\Image{figures/part_completion/chairs/9.png}
\Image{figures/part_completion/chairs/12.png}
\Image{figures/part_completion/chairs/62.png}
\Image{figures/part_completion/chairs/97.png}
\Image{figures/part_completion/chairs/107.png}
\Image{figures/part_completion/chairs/126.png}
\Image{figures/part_completion/chairs/135.png}
\Image{figures/part_completion/chairs/136.png}
\Image{figures/part_completion/chairs/153.png}
\Image{figures/part_completion/chairs/148.png}
% \Image{figures/part_completion/chairs/181.png}
% \Image{figures/part_completion/chairs/190.png}
% \Image{figures/part_completion/chairs/203.png}
% \Image{figures/part_completion/chairs/234.png}




==> figures/part_completion/supp_part_completion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\CatchFileDef{\AllComparisonImages}{figures/part_completion/chair_list.tex}{}
% \graphicspath{{figures/shape_generation/}}

\makeatletter
\def\Image#1{%
  \multicolumn{\LT@cols}{l}{\includegraphics[width=\textwidth]{#1}}\\
}
\makeatother
{
\setlength{\tabcolsep}{0em}
\def\arraystretch{0.0}
\renewcommand\tabularxcolumn[1]{m{#1}}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcolumntype{W}{>{\centering\arraybackslash}m{0.1111\textwidth}}
\newcolumntype{Z}{>{\centering\arraybackslash}m{0.2222\textwidth}}
{\scriptsize
\begin{longtable}{WWW|Z|Z|Z}
GT & Bounding Box & Gaussians & ShapeFormer~\cite{Yan:2022ShapeFormer} & Neural Wavelet~\cite{Hui:2022NeuralWavelet} & \salad{} (Ours) \\ 
  \midrule
  \endhead

  \bottomrule
  \endfoot

  \AllComparisonImages
\end{longtable}
}

\CatchFileDef{\AllComparisonImages}{figures/part_completion/airplane_list.tex}{}
% \graphicspath{{figures/shape_generation/}}

\makeatletter
\def\Image#1{%
  \multicolumn{\LT@cols}{l}{\includegraphics[width=\textwidth]{#1}}\\
}
\makeatother
{
\setlength{\tabcolsep}{0em}
\def\arraystretch{0.0}
\renewcommand\tabularxcolumn[1]{m{#1}}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcolumntype{W}{>{\centering\arraybackslash}m{0.1111\textwidth}}
\newcolumntype{Z}{>{\centering\arraybackslash}m{0.2222\textwidth}}
{\scriptsize
\begin{longtable}{WWW|Z|Z|Z}
GT & Bounding Box & Gaussians & ShapeFormer~\cite{Yan:2022ShapeFormer} & Neural Wavelet~\cite{Hui:2022NeuralWavelet} & \salad{} (Ours) \\ 
  \midrule
  \endhead

  \bottomrule
  \endfoot

  \AllComparisonImages
\end{longtable}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table class part completion figure %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[h!]
% \centering
% {
% \scriptsize
% \def\arraystretch{0.0}
% \setlength{\tabcolsep}{0em}
% \renewcommand\tabularxcolumn[1]{m{#1}}
% \newcolumntype{W}{>{\centering\arraybackslash}m{0.125\textwidth}}
% \newcolumntype{Z}{>{\centering\arraybackslash}m{0.25\textwidth}}
% \begin{tabularx}{\textwidth}{WWZ|WWZ }
% GT & Gaussians & \salad{} (Ours) & GT & Gaussians & \salad{} (Ours) \\
% \multicolumn{6}{c}{\includegraphics[width=\textwidth]{figures/part_completion/tables/fig-0.png}}\\
% \multicolumn{6}{c}{\includegraphics[width=\textwidth]{figures/part_completion/tables/fig-1.png}}\\
% \multicolumn{6}{c}{\includegraphics[width=\textwidth]{figures/part_completion/tables/fig-2.png}}\\
% \multicolumn{6}{c}{\includegraphics[width=\textwidth]{figures/part_completion/tables/fig-3.png}}\\
% \multicolumn{6}{c}{\includegraphics[width=\textwidth]{figures/part_completion/tables/fig-4.png}}\\
% \multicolumn{6}{c}{\includegraphics[width=\textwidth]{figures/part_completion/tables/fig-5.png}}
% \end{tabularx}
% }
% \end{figure*}
% }

==> figures/shape_completion.tex <==
\setlength{\tabcolsep}{0em}
\def\arraystretch{0.0}
%\newcolumntype{Y}{>{\centering\arraybackslash}m{0.0909\textwidth}}
\begin{figure*}
{\scriptsize
\begin{tabularx}{\linewidth}{YYYYYYYYY}
GT & \makecell{Bounding \\box}  Gaus. & \multiolumn{2}{c}{ShapeFormer} & \multicolumn{2}{c}{Neural Wavelet} & \multicolumn{2}{c}{Ours} \\  
\midrule
\multicolumn{9}{c}{\includegraphics[width=\linewidth]{figures/fig2_chair.png}} \\
\multicolumn{9}{c}{\includegraphics[width=\linewidth]{figures/fig2_airplane.png}} 
\end{tabularx}
}
\caption{Ablation studies.}
\label{fig:ablation_study}
\vspace{-0.5\baselineskip}
\end{figure*}

==> iccv2023AuthorKit/old/1_Introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}

% What is the motivation of your research (not your personal motivation, but why is it needed and important in the academia/industry?)
% Why 3D generative model being capable of generating and manipulating shapes is important.
% don't mention generative models here. focus on creation that includes generation and editing instead of generation only.
\Juil{start with TL;DR.} Leaving the realm of creation to machines has long been studied. Creating assets requires considerable effort and time. In particular, as the demand for processing 3D data has been prevalent across various fields, such as computer vision, computer graphics, robotics, and the metaverse, it has become more important to reduce the cost required to generate a new 3D asset or to edit the existing asset. 
% In response to 
To address this, previous work~\cite{Achlioptas:2018latentgan, Hao:2020Dualsdf, Chen:2019ImNet, Yin:2020Coalesce} has proposed various methods, mainly focusing only on either shape generation or manipulation. 
%However, it is still challenging to achieve both high fidelity and editability in handling 3D assets. 
However, achieving high-fidelity generation while still allowing 3D assets to be editable remains a challenge. 
To democratize the creation of 3D assets, it is essential to enhance not only a high-fidelity generation but also an interpretable shape manipulation. 

%Diffusion: good generation results. also inherently capable of editing or synthesizing input data.
% shorten content of other generative models. directly say about diffusion models. emphasize diffusion model characteristics: zero-shot editing capability to unseen images. SDEdit, etc.
The recent advance of diffusion models~\cite{Ho:2019DDPM, Dhariwal:2021DiffusionBeatGANs} has led to significant growth in the 2D image generation, subsequently replacing the existing generative models~\cite{Goodfellow:2014GAN, Kingma:2014VAE, Rezende:2015Flow} with superior performance. The key advantage of diffusion models compared to other generative models is they have shown a zero-shot capability of editing and synthesizing input data. Without any supervision or context of task-specific conditions during training, its prior has demonstrated a capability of image inpainting~\cite{Lugmayr:2022Repaint, Chung:2022MCG} and image synthesis~\cite{Meng:2022SDEdit}. These attractive characteristics and the ability of diffusion models in the 2D image domain have prompted attempts to apply diffusion models to the 3D generation task.

% 3D data representation
% first paragraph: low-quality of early work
% second paragraph: difficulty of manipulating 3d data in previous work
Much previous work~\cite{Li:2022Diffusion-Sdf, Chou:2022Diffusionsdf, Shue:2022TriplaneDiffusion, Cheng:2022SDFusion, Hu:2023NeuralWavelet, Hui:2022NeuralWavelet, Cai:2020ShapeGF, Luo:2021DPM, Zeng:2022LION} has introduced diffusion models for 3D generation task. Early work of the literature employs diffusion models with 3D point clouds~\cite{Cai:2020ShapeGF, Luo:2021DPM, Zeng:2022LION} or a point-voxel hybrid representation~\cite{Zhou:2021PVD}, since na\"ively adopting 2D diffusion models to 3D voxels would require orders of magnitude more computational power. However, these early attempts fail to capture detailed shape surfaces due to the inherent limitation of shape\Charlie{pointcloud} representation, thus producing low-quality results. In addition, although they can convert output point clouds to iso-surface meshes, it requires another post-processing where a very precise computation is necessary. Otherwise, it is prone to produce noisy artifacts. 

To obtain high resolution meshes using 3D diffusion models, concurrent work~\cite{Li:2022Diffusion-Sdf, Chou:2022Diffusionsdf, Cheng:2022SDFusion, Hui:2022NeuralWavelet, Hu:2023NeuralWavelet} has introduced %3D implicit function-based diffusion models. 
diffusion models based on implicit function.
To mitigate the high computational cost of running diffusion on high-resolution 3D voxels, they run diffusion on intermediate feature space. Albeit showing local shape manipulation using the intermediate latent space, it is still non-trivial for users to select local regions from the latent space, thus limiting them from even the simplest manipulation capability.
% I will edit before this line.

% SALAD explanation: shape representation and strengths
% remove all notations. explain in English.
% synergy between diffusion models and our representation.

To resolve the aforementioned issues, we propose a 3D \textbf{S}hape P\textbf{A}rt-Level \textbf{LA}tent \textbf{D}iffusion Model, called \textbf{SALAD}. When designing a new 3D generative model, the \emph{desiderata} we consider is first, it should produce diverse and realistic meshes, and it also should provide users with a straightforward shape manipulation method. Inspired by Hertz~\etal~\cite{Hertz:2022Spaghetti} who has introduced a part-level shape representation, we observe the synergy between diffusion models and a part-level shape representation. Diffusion models present high-quality generations as well as a zero-shot capability of input synthesis, and the part-level shape representation decomposes a complex 3D shape into a set of simple parts. We demonstrate that the key ingredients of aiding 3D asset creation, high fidelity generation, intuitive shape manipulation, and completion, are only available when a diffusion model and a part-level representation are combined. 

SALAD is a latent diffusion model based on a set of part-level shape latents consisting of a 3D shape. The part latents can represent a high-resolution 3D mesh with significantly fewer entities than point clouds. Furthermore, each part latent affects only the local region where it governs in the 3D space. Its locality enables part-level shape manipulation and completion.
Since our shape representation is defined as a set, we use Transformer~\cite{Vaswani:2017Attention} architecture to address the permutation invariance of the part latents. Also, inspired by Ho~\etal~\cite{Ho:2022CascadedLDM}, we propose a two-phase training process, which is another crucial detail of the training. This training strategy splits the amount of information the model learns into two phases, thus making the training more stable and easier. Instead of running diffusion at once in a high-dimensional latent space, we separate the latent space into two sub-spaces. More precisely, we first train an unconditional latent diffusion model with a low dimensional latent which captures rough geometry information of a 3D space with a few parameters. Finally, to fill in the remaining detailed information for a final shape, we train another conditional latent diffusion model on the other latent space leveraging the low dimensional latent as a condition. Figure~\ref{fig:teaser} shows a coarse structure captured by the low-dimensional latents and its corresponding final decoded 3D shape. 

The effectiveness of our training strategy is demonstrated in Table~\ref{tbl:quantitative_comparison_of_shape_generation} which shows a big improvement. In addition, we demonstrate SALAD is suitable for various applications including part-level shape manipulation, shape completion, and conditional generation. In summary, the following are our contributions:
\begin{itemize}
    \item We introduce SALAD which generates diverse and high-resolution meshes with significantly less memory and computation. Quantitatively, we show that SALAD outperforms other baselines in random shape generation.
    \item Our SALAD is capable of part-level shape manipulation, which enables various applications, such as part-level shape manipulation, completion, and language-conditioned manipulation.
\end{itemize}


% Recently, as the demand of processing 3D contents has been growing in various fields, such as meta-verse, robotics, computer vision, and computer graphics, coupled with the difficulty of handling 3D data, a 3D generative model that not only generates high quality shapes but also enables users to easily manipulate the 3D shapes has been required. However, most of previous 3D generative model research has focused on generation quality itself only.

% At the same time, as diffusion models~\cite{Dhariwal:2021DiffusionBeatGANs} have outperformed other existing generative models~\cite{Goodfellow:2014GAN, Kingma:2014VAE, Rezende:2015Flow} in the 2D image and audio domain, attempts to apply a diffusion model on 3D shapes have been introduced in various previous works~\cite{Chou:2022Diffusionsdf, Hui:2022NeuralWavelet, Li:2022Diffusion-Sdf, Zhou:2021PVD, Luo:2021DPM, Jiang:2020Shapeflow}. However, unlike 2D images, there is no standard 3D representation, querying which 3D representation is the most efficient in 3D shape generation. In response to the question, we propose a 3D \textbf{S}hape P\textbf{A}rt-level \textbf{LA}tent \textbf{D}iffusion Model, called \textbf{SALAD}, which provides straightforward local part editing capability with diverse and high-quality 3D generated shapes.  

% Our model is based on part-level latents, which is the most efficient 3D representation compared to other representations, such as point clouds, voxels, and meshes. A 3D shape is encoded to a set of part latents $\{\Vp_j\}$, which represents the shape with a much smaller number than point clouds and voxels. Each $\Vp_j$ is further separated into an extrinsic latent $\Ve_j$ and an intrinsic latent $\Vs_j$. \Juil{need to flesh out descriptions of the role of each latent.} Instead of learning a distribution of these latents at once, inspired by cascaded LDM~\cite{Ho:2022CascadedLDM}, we split the LDM training into two phases. In the first phase, we first model a distribution of $\{\Ve_j\}$ which represents a rough geometry structure of input shape without any surface details. Next, the second phase model learns a conditional distribution of $\{\Vs_j\}$ given $\{\Ve_j\}$, which corresponds to filling in detailed 3D surface information given the rough geometry. 
% We use Transformer~\cite{Vaswani:2017Attention} architecture on both phase 1 and phase 2 latent diffusion models which is suit for processing set data.
% In test time, sampled $\{\Ve_j\}$ and $\{\Vs_j\}$ are decoded to an implicit representation, which can be easily converted to a mesh, by a pre-trained implicit decoder $\mathcal{D}$. 

% We demonstrate our two-phase design is crucial to produce high-quality 3D shapes and two-level shape manipulation, overall modification with coarse structure $\{\Ve_j\}$, and fine customizing with $\{\Vs_j\}$. \Juil{argument of two-level shape manipulation doesn't seem to make sense considering our results..} 

% \Seungwoo{It would be good to summarize our contribution in several bullets}

% What is the limitation of previous work?
% -> Unlike 2D images, there is no standard representation. 
% -> Most of 3d generative models have focused on generation quality itself only.

% What is the exact problem setup of your work?
% -> Encode a 3D shape to part-level latents which are further separated to extrinsic and intrinsic latents.
% -> Instead of learning a distribution of these latents at once, inspired by cascaded LDM, we design a cascaded latent diffusion model.
% -> In the first phase, we first model a distribution of extrinsic latents which represents a rough geometry structure without any surface details.
% -> Next, our second phase model learns a conditional distribution of intrinsic given input extrinsics, which means the phase 2 model produce detailed surface information given the rough geometry.
% -> We demonstrate our two-phase design outperforms a single phase model that models data distribution of extrinsic and intrinsic at the same time.

% What is the key challenge to solving the problem?
% -> simple single-phase model doesn't work. our two phases setup is crucial for high quality generation.
% -> Transformer architecture is essential in modeling set representation. 

% A list of contributions you aim for.
% -> We first propose a diffusion model for 3D shape generation and straightforward local part "manipulation".

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VERSION 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In 3D data, data representation is important. ours is the best.
% Unlike 2D images, 3D data has no standard data representation. 


% In recent, modeling and manipulating 3D shapes have become more prevalent in various fields, such as robotics, computer vision, computer graphics, and the Metaverse, where it is common to process 3D data. Coupled with the difficulty of handling 3D data, the need for a 3D generative model capable of generating high-quality shapes as well as manipulating the shapes is increasing. In response to this, much previous work~\cite{Li:2022Diffusion-Sdf, Chou:2022Diffusionsdf, Shue:2022TriplaneDiffusion, Cheng:2022SDFusion, Hu:2023NeuralWavelet, Hui:2022NeuralWavelet, Cai:2020ShapeGF, Luo:2021DPM, Zeng:2022LION} has introduced diffusion models for 3D generation task. Na\"ively adopting 2D diffusion models directly to 3D voxels would require orders of magnitude more computational power. Thus, early work employs diffusion models with 3D point clouds~\cite{Cai:2020ShapeGF,Luo:2021DPM,Zeng:2022LION} or a point-voxel hybrid representation~\cite{Zhou:2021PVD}. However, this straightforward approach failed to capture detailed shape surface information and produce low-quality results. To resolve this, concurrent work~\cite{Li:2022Diffusion-Sdf,Chou:2022Diffusionsdf, Cheng:2022SDFusion, Hui:2022NeuralWavelet, Hu:2023NeuralWavelet} has attempted applying diffusion models to a 3D implicit function representation by running diffusion on intermediate latent space or wavelet-domain. Albeit achieving higher quality generation, Diffusion-SDF~\cite{Li:2022Diffusion-Sdf}, Neural Wavelet~\cite{Hui:2022NeuralWavelet, Hu:2023NeuralWavelet}, and SDFusion~\cite{Cheng:2022SDFusion} are still relatively computationally heavy since they use down-sampled 3D grid features. Another problem with these voxel-based representations is that they are 
% inherently difficult to manipulate. In particular, it is not trivial to select local regions in the representation that DiffusionSDF~\cite{Chou:2022Diffusionsdf} and Neural Wavelet~\cite{Hui:2022NeuralWavelet, Hu:2023NeuralWavelet} provide, and thus limiting them from even the simplest manipulation capability.

% To resolve all the aforementioned issues, we propose a 3D \textbf{S}hape P\textbf{A}rt-Level \textbf{LA}tent \textbf{D}iffusion Model, called \textbf{SALAD}, which is capable of manipulating and generating high-quality and diverse 3D shapes at a part level while costing significantly less memory and computation. Our model utilizes part-level latents that ensure local influence in a 3D shape and are disentangled to extrinsic properties and intrinsic properties. 

% Let a 3D shape be encoded to a set of part latents $\{\Vp_j\}_{j=1}^M$, where $M$ denotes the number of parts representing the shape. Each $\Vp_j$ is further separated into an extrinsic latent $\Ve_j$ and an intrinsic latent $\Vs_j$. Intuitively, $\Ve_j$ encapsulates basic geometric information of a local part and consists of a few parameters. Figure~\ref{fig:teaser} shows a coarse structure that $\{\Ve_j\}$ captures and the decoded 3D shape. On the other hand, the higher dimensional vector $\Vs_j$ captures detailed surface information as well as joint regions between the parts. This set of latents are then decoded to a 3D shape by an implicit decoder $\mathcal{D}$:
% \begin{equation}
% \begin{aligned}
%     o=\mathcal{D}(\mathbf{x} | \{\Ve_j\},\, \{\Vs_j\}),
% \end{aligned}
% \end{equation}
% where $\mathbf{x}\in\Real^3$ and $o\in [0,1]$ denote a query 3D point and its corresponding occupancy value, respectively. 
% Unlike 3D voxel-based diffusion models~\cite{Li:2022Diffusion-Sdf, Chou:2022Diffusionsdf, Cheng:2022SDFusion, Hui:2022NeuralWavelet, Hu:2023NeuralWavelet}, our shape representation is a set representation which is invariant to the permutation of its elements. Inspired by Lee~\etal~\cite{Lee:2019SetTF}, we guarantee this property by adopting Transformer~\cite{Vaswani:2017Attention}, which is permutation invariant, to our latent diffusion models. Unlike previous point cloud-based diffusion models~\cite{Cai:2020ShapeGF, Luo:2021DPM} ~\Juil{Not sure if LION also doesn't use self-attention.}that uses point-wise feed-forward layers, we demonstrate that the self-attention module is a crucial architecture design for a diffusion model with a small number of elements as ours only used 16 part-latents. Inspired by Ho~\etal~\cite{Ho:2022CascadedLDM}, another key detail in our diffusion model design is to split a training process into two phases that each tailored to leverage the idiosyncrasy of the extrinsic and intrinsic representation. We first train an unconditional latent diffusion model with $\{\Ve_j\}$ which predicts noises in the $\Ve_j$ latent space. It corresponds to modeling a distribution of rough geometry of training shapes. In the second phase, we train a \emph{conditional} latent diffusion model which learns a conditional distribution $p(\Vs_j | \Ve_j)$. The latter model predicts noises in the $\Vs_j$ latent space with given condition $\Ve_j$. Splitting allows the first phase to learn only rough geometry of training shapes which reduce the complexity of the model significantly compared to previous methods. This ease of learning also allows the first phase model to create a much more diverse set of output. The second can then take advantage of this information to produce higher quality output. Altogether, we were able to achieve high fidelity in shape generation with higher variation while keeping the computational footprint low. We experimentally demonstrate the advantage of this split training approach by comparing against other model architectures. 

% To generate 3D models at test time, we first randomly sample $\{\hat{\Ve}_j\}$ from the first phase model. Then, we sample $\{\hat{\Vs}_j\}$ by feeding ${\{\hat{\Ve}_j\}}$ as condition to the second phase model. From these sampled latents, we obtain the final shape through the pre-trained Decoder $\mathcal{D}$. Since $\{\Ve_j\}$ represents a 3D shape as a primitive set and its variation affects the final output shape, our method also allows user to directly perform part editing method with minimal effort similarly to previous primitive-based shape representation work~\cite{Hao:2020Dualsdf, Hertz:2022Spaghetti}. Compared to previous methods, we also demonstrate that SALAD is the most suitable 3D generative model as it allow part-level shape manipulation, completion, and conditional shape generation. 

% In summary, the following are our contributions:
% \begin{itemize}
%     \item We first introduce a part-level latent diffusion model, SALAD, which generates diverse and high-resolution meshes with significantly less memory and computation. Quantitatively, we show that SALAD outperforms other baselines in random shape generation.
%     \item We present a Transformer-based network that enables a diffusion model training when a small number of elements is given.
%     \item We propose a cascaded training strategy for 3D generation and experimentally demonstrate its effectiveness.
%     \item To our best knowledge, SALAD is the first 3D diffusion model to provide primitive-based shape manipulation. Unlike previous work~\cite{Li:2022Diffusion-Sdf, Cheng:2022SDFusion, Hu:2023NeuralWavelet, Hui:2022NeuralWavelet}, it enables users to intuitively select and edit local regions. 
% \end{itemize}


==> iccv2023AuthorKit/old/2_Related_Work_old.tex <==
\section{Related Work}
\label{sec:related_work}

%==== Keypoints ====%

%List related papers with a BibTeX reference and a tl’dr (a description with a few sentences). Try to classify the papers into 2-3 categories. Keep adding papers.

%==================

%We briefly overview the literature related to our work in the followings, focusing on generative modeling for 3D shapes and part-level 3D representations.

% \Seungwoo{TODO: Briefly introduce GAN-based generative models in the first few sentences and start introducing diffusion-based works in details}
\paragraph{3D Generative Models.}

% \Seungwoo{Add other types of models such as AR, Flow, Energy-based, etc}
% There have been continual efforts to model distributions of 3D shapes in various representations. 
% \Seungwoo{GAN and VAE based method produces unsatisfying results}
% There have been continual efforts to model distributions of 3D shapes by leveraging generative modeling frameworks~\cite{Goodfellow:2014GAN,Rezende:2015NF,Van:2016Pixel,Van:2016WaveNet} that are widely adapted in other domains. 
There have been continual efforts to model distributions of 3D shapes by adapting various frameworks, such as GAN~\cite{Goodfellow:2014GAN}, Normalizing Flows~\cite{Rezende:2015NF}, or autoregressive models~\cite{Van:2016Pixel,Van:2016WaveNet}, that are widely studied in other domains.

A branch of work leverage GAN~\cite{Goodfellow:2014GAN} and learn distributions of latents that are decoded into various 3D representations including point clouds~\cite{Achlioptas:2018LatentGAN,Valsesia:2019GraphConv,Shu:2019Treegan} and implicit representations~\cite{Kleineberg:2020VoxelGAN,Hao:2020Dualsdf,Chen:2019ImNet,Ibing:2021GridBased}. This approach has been popular until recently, as represented in several work~\cite{Chan:2022EG3D,Gao:2022Get3d} that extend StyleGAN~\cite{Karras:2020StyleGAN2} further by combining its network architecture and differentiable renderer~\textbf{cite!}.

% Zheng:2022SdfStylegan
% Zheng:2022SdfStylegan,Gao:2022Get3d

%%%% Looks like OccNet uses VAE not GAN \cite{Mescheder:2019OccNet}

Another line of work instead build on autoregressive models~\cite{Van:2016Pixel,Van:2016WaveNet} to generate 3D shapes in  forms of meshes~\cite{Nash:2020Polygen}, point clouds~\cite{Sun:2020PointGrow}, or (ir)regular feature grids~\cite{Zhang:20223DILG,Yan:2022ShapeFormer}. They demonstrate their efficiacy in a wide range of downstream tasks, such as shape reconstruction and completion, but also in multi-modal conditional generation~\cite{Mittal:2022Autosdf,Fu:2022Shapecrafter}.

% Concurrently, approaches~\cite{Nash:2020Polygen,Sun:2020PointGrow,Zhang:20223DILG,Yan:2022ShapeFormer} that stem from autoregressive models~\cite{Van:2016Pixel,Van:2016WaveNet} deliver impressive results and extend themselves to a wider range of applications such as multi-modal 3D shape generation~\cite{Mittal:2022Autosdf,Fu:2022Shapecrafter}. % Furthermore, a distribution of work based on other types of framework, such as Normalizing Flows~\cite{Yang:2019PointFlow}, also 

% Achlioptas~\etal~\cite{Achlioptas:2018latentgan}, Valsesia~\etal~\cite{Valsesia:2019graph}, and Shu~\etal~\cite{Shu:2019treegan} propose generative models for point clouds based on GAN~\cite{Goodfellow:2014GAN} whereas Mescheder~\etal~\cite{Mescheder:2019OccNet}, Chen~\etal~\cite{Chen:2019ImNet}, Ibing~\etal~\cite{Ibing:2021GridBased}, Kleineberg~\etal~\cite{Kleineberg:2020VoxelGAN}, Hao~\etal~\cite{Hao:2020Dualsdf}, Zheng~\etal~\cite{Zheng:2022SdfStylegan}, and Gao~\etal~\cite{Gao:2022Get3d} 


% For instance, frameworks based on GAN~\cite{Goodfellow:2014GAN} demonstrated their capability of modeling distributions of point clouds~\cite{Achlioptas:2018latentgan,Valsesia:2019graph,Shu:2019treegan}, voxels~\cite{Smith:2017IWGAN}, and implicit functions~\cite{Kleineberg:2020VoxelGAN,Hao:2020Dualsdf,Zheng:2022SdfStylegan,Gao:2022Get3d,Mescheder:2019OccNet,Chen:2019ImNet,Ibing:2021GridBased}.
% There have been continual efforts to model distributions of 3D shapes in various representations. For instance, frameworks based on GAN~\cite{Goodfellow:2014GAN} demonstrated their capability of modeling distributions of point clouds~\cite{Achlioptas:2018latentgan,Valsesia:2019graph,Shu:2019treegan}, voxels~\cite{Smith:2017IWGAN}, and implicit functions~\cite{Kleineberg:2020VoxelGAN,Hao:2020Dualsdf,Zheng:2022SdfStylegan,Gao:2022Get3d,Mescheder:2019OccNet,Chen:2019ImNet,Ibing:2021GridBased}. While such approaches gained success in the field, they also suffered from several problems, such as training instability, that mostly originate from adversarial training.

% \Seungwoo{diffusion based model can be directly applied to 3D data, producing satisying results at the same time.}
% Recently, a line of work started to employ the core idea from diffusion models~\cite{Ho:2019DDPM} and score-based models~\cite{Song:2019Score} to achieve better generation quality. 
As of now, the major interest of the literature has moved to recent breakthroughs in 2D generative modeling, represented by diffusion models~\cite{Ho:2019DDPM} and score-based models~\cite{Song:2019Score}. Specifically, Cai~\etal~\cite{Cai:2020ShapeGF}, Luo~\etal~\cite{Luo:2021DPM}, and Zhou~\etal~\cite{Zhou:2021PVD} propose score-based~\cite{Cai:2020ShapeGF} or diffusion-based~\cite{Luo:2021DPM,Zhou:2021PVD} pipeline for learning distributions of point clouds. Hui~\etal~\cite{Hui:2022NeuralWavelet} adapts voxel grids of wavelet coefficients~\cite{Mallat1989:Wavelet,Daubechies1990:Wavelet,Velho1994:Wavelet} as compact representations of truncated signed distance functions (TSDFs) for diffusion models. Furthermore, the recent success of latent diffusion models (LDMs)~\cite{Rombach:2022LDM} in 2D image domain has prompted development of diffusion models operating in latent spaces of 3D representations, including triplanes~\cite{Shue:2022TriplaneDiffusion}, latent point clouds~\cite{Zeng:2022LION}, latent voxels~\cite{Li:2022Diffusion-Sdf}, or VAE~\cite{Kingma:2014VAE} embeddings~\cite{Chou:2022Diffusionsdf}.
\Seungwoo{They are not just latent diffusion models, but take spatial prior into account when introducing such latents}

% However, we emphasize that none of the aforementioned work allows for intuitive editing of 3D shapes due to inherent limitations of their 3D representations.
\Seungwoo{Less aggressive tone.}
However, we emphasize that none of the aforementioned work delivers both high-quality and editable shapes due to inherent limitations of their 3D representations.
% as their shape representations inherently lack support for local controls. % or do not provide spatial, geometric interpretation of latent features.
This raises the problem of finding an appropriate alternative that (\num{1}) is compact enough for diffusion-based pipeline, and (\num{2}) disentangles 3D shapes into several components to make manipulation easier. Therefore, we opt to explore previous work focusing on formulating part-level interpretations of 3D shapes.

%\paragraph{3D Shape Representation.}
\paragraph{Part-Level 3D Representation.}
Decomposing a complex subject into smaller components helps human get better understanding of its essence, and this is not an exception for 3D shapes. For instance, early work~\cite{} in computer vision proposed to fit simple primitives, such as cuboids~\cite{}, to 3D shapes for various cognitive tasks involving understanding of 3D geometry. The same rationale can be found in recent work aiming to devise better decomposed representations based on volumetric primitives~\cite{volumetric primitives}, quadrics~\cite{superquadric}~, or convexes~\cite{Chen:2020BspNet,CvxNet}. Although primitive-based decompositions produce more compact representations, they partition geometry as is, which can be still challenging to manipulate or edit.

% On the other hand, the success of neural implicit functions~\cite{Park:2019Deepsdf,Mescheder:2019OccNet} hinted their potential as 3D representations that are suitable for learning-based framework. While such representations are agnostic to sampling resolution and thus can convey high-frequency details, they lack editability as a 3D shape is approximated with a single analytic function. This motivated a body of work that focus on factoring out or 
Similarly, while the success of neural implicit functions~\cite{Park:2019Deepsdf,Mescheder:2019OccNet} hinted their potential as 3D representations that are suitable for learning-based framework, they also lack editability as a 3D shape is approximated with a single analytic function. Their limitation has motivated a body of work focusing on factoring out implicit function into several local components~\cite{Genova:2019LearningShapeTemplates,Genova:2020LDIF,Hertz:2022Spaghetti}, or separating topology information from local geometry~\cite{Hui:2022NeuralTemplate}. \Seungwoo{More detailed description on LDIF and Neural Templates..?} In particular, Hertz~\etal~\cite{Hertz:2022Spaghetti} propose to model overall structure of 3D shapes as Gaussian Mixture Models (GMMs) and to encode local geometry into latent codes, thereby enable various application such as local editing and part mixing.
\Seungwoo{One liner emphasizing the use of such part-level representation! In accordance with intro and background.}

Decomposing 3D shapes into multiple parts 

Decomposed representations for 3D shapes 

% Genova~\etal~\cite{Genova:2020LDIF} proposes to decompose a 3D shape into multiple shape elements that, together with a query point, can be decoded to values of a implicit function.
% Hui~\etal~\cite{Hui:2022NeuralTemplate} introduces a topology-aware representation consisting of two latent codes that disentangles overall shape topology from detailed geometry.
% Similarly, Hertz~\etal~\cite{Hertz:2022Spaghetti} decouples global structure and local geometry 

% Local Deep Implicit Functions (LDIF)~\cite{Genova:2020LDIF}. 
% Hao~\etal~\cite{Hao:2020Dualsdf} proposes a joint latent of a fine-grained detail shape and its primitive-based coarse proxy shape where the shape can be manipulated by moving primitives.
% Hui~\etal~\cite{Hui:2022NeuralTemplate} proposes two disentangled shape latent codes, one determines the topolgy of a shape and the other refines the rough template shape.
% SPAGHETTI~\cite{Hertz:2022Spaghetti} proposes to learn disentangled representations for 3D, and allows for sampling from the learned shape prior distribution. The disentangled part representation allow user to deform the final shape by apply affine transformations on the corresponding Gaussian primitives.  

% In particular, GAN-based approaches~\cite{Achlioptas:2018latentgan, Shu:2019treegan, Kleineberg:2020VoxelGAN} had form the mainstream in the field. 

% In particular, approaches based on the adversarial loss introduced in Goodfellow~\etal~\cite{Goodfellow:2014GAN} had formed the mainstream in the field. 3D representations of their choice include point clouds~\cite{Achlioptas:2018latentgan,Valsesia:2019graph,Shu:2019treegan}, voxels~\cite{Smith:2017IWGAN}, signed distance functions~\cite{Kleineberg:2020VoxelGAN,Hao:2020Dualsdf,Zheng:2022SdfStylegan,Gao:2022Get3d}, occupancy fields~\cite{Mescheder:2019OccNet,Chen:2019ImNet,Ibing:2021GridBased}, or meshes~\cite{Luo:2021SurfGen}. However, the interest of research community has made a gradually transition to diffusion models~\cite{Ho:2019DDPM}, or score-based models~\cite{Song:2019Score}, after witnessing their success in modeling distributions of 2D images. As our work is more relevant to the previous work of this class, we focus on surveying the literature in details.

% \paragraph{Diffusion Models for 3D Data.}
% Similar to 3D generative frameworks based on GAN~\cite{Goodfellow:2014GAN}, diffusion models~\cite{Ho:2019DDPM}, or score-based models~\cite{Song:2019Score}, for 3D data have been actively developed upon various 3D representations including point clouds~\cite{Cai:2020ShapeGF,Luo:2021DPM,Zhou:2021PVD,Zeng:2022LION}, implicit representations~\cite{Shue:2022TriplaneDiffusion,Li:2022Diffusion-Sdf,Hui:2022NeuralWavelet}, and meshes~\cite{Liu:2023MeshDiffusion}. Furthermore, recent work~\cite{Zeng:2022LION,Chou:2022Diffusionsdf} propose diffusion models operating in learned latent spaces of the previously mentioned 3D representations, inspired by the success of latent diffusion models (LDMs)~\cite{Rombach:2022LDM} in image domain.

% Cai~\etal~\cite{Cai:2020ShapeGF}, Luo~\etal~\cite{Luo:2021DPM}, and Zhou~\etal~\cite{Zhou:2021PVD} view points in point clouds as particles either (\num{1}) traversing along density gradient fields~\cite{Cai:2020ShapeGF} or (\num{2}) dissipating under thermodynamic systems~\cite{Luo:2021DPM,Zhou:2021PVD} and propose to train neural networks that reverse such processes.
%Such methods take point clouds as inputs that require network architectures~\cite{Qi:2017Pointnet} capable of handling permutation invariant data.
% While point clouds can effectively represent the overall structure of 3D shapes, they cannot capture fine details of the underlying geometry as their expressiveness greatly depends on the sampling resolution.

% More importantly, these models' inputs are order-invariant, unlike images, point clouds are equivalent with respect to permutation. More recently, Liu \etal~\cite{Liu:2023MeshDiffusion} introduces MeshDiffusion that directly trained on mesh-grid. 

% Another work model distributions of implicit functions, particularly signed distance functions (SDFs)~\cite{Hui:2022NeuralWavelet}. Compared to point clouds, implicit functions are capable of capturing high-frequency details of 3D shapes, and thus widely studied in learning-based approaches~\cite{Park:2019Deepsdf,Mescheder:2019OccNet} that aim to devise compact, resolution-agnostic representations for 3D shapes. However, such representations are often realized as voxel grids with function values at each cell, which make them less intriguing for diffusion-based generative modeling due to high computational cost. Hui~\etal~\cite{Hui:2022NeuralWavelet} alleviate this issue by learning a diffusion model on wavelet coefficients of truncated signed distance functions (TSDFs) derived via wavelet transform~\cite{Velho1994:Wavelet,Daubechies1990:Wavelet,Mallat1989:Wavelet}. Although it produces impressive results, such a representation does not provide direct control over local regions. % \Seungwoo{Refine this line more.}

% A body of work that also deserve our attention focus on building diffusion models for latent features of the aforementioned representations~\cite{Shue:2022TriplaneDiffusion,Li:2022Diffusion-Sdf,Chou:2022Diffusionsdf,Zeng:2022LION}. LION~\cite{Zeng:2022LION} employs a hierarchical latent space of point clouds which comprises two latent spaces of global shape features and per-point features, respectively. Shue~\etal~\cite{Shue:2022TriplaneDiffusion} suggest a method based on axis-aligned triplane features obtained by factorizing occupancy grids, whereas Chou~\etal~\cite{Chou:2022Diffusionsdf} employs a two-stage training pipeline that consists of VAE~\cite{Kingma:2014VAE} encoding latents of 3D shapes and a diffusion model which operates on the learned latent space. \Seungwoo{However, latent diffusion models are also struggle on tasks involving local editing... in a more neat sentence!}

% Another work in diffusion on SDF representation is Diffusion-SDF~\cite{Li:2022Diffusion-Sdf}.  Li~\etal~\cite{Li:2022Diffusion-Sdf} leverages a text-conditioned, diffusion model to learn the distribution of 3D shapes represented by truncated sign distance fields (TSDF). Instead of training directly on the spatial domain of TSDF, Hui~\etal~\cite{Hui:2022NeuralWavelet} proposes a two step diffusion pipeline where the distribution of compact coarse wavelet coefficient voxels is learned through a diffusion model and a secondary diffusion model is trained to then generate the detailed wavelet coefficients. 

% Inspired by the success of latent diffusion models (LDMs)~\cite{Rombach:2022LDM} in image domain, a more recent work~\cite{Zeng:2022LION} proposes a framework that consists of variational autoencoders (VAEs)~\cite{Kingma:2014VAE} and diffusion models~\cite{Ho:2019DDPM} operating in the learned, hierarchical latent space.
% diffusion on latent space. Decode to SDF, PointCloud
% There were also hybrid approaches in using diffusion model on mixed explicit representation and neural network's latents.
% Chou~\etal~\cite{Chou:2022Diffusionsdf} employs a two-stage training pipeline that consists of VAE encoding latents of 3D shapes and a diffusion model which operates on the learned latent space. LION~\cite{Zeng:2022LION} also have additional latent information for each point in pointcloud representation.

% diffusion on image space, backprop to density field, voxel
% \Seungwoo{Why referring to NeRFs...?}
% Concurrent work on NeRF~\cite{Mildenhall:2020NeRF} have shown that  diffusion model trained on image space could be distilled to neural renders. DreamFusion~\cite{Poole:2023Dreamfusion} extends on Dream Fields~\cite{Jain:2022DreamFields} by using Score Distillation Sampling loss as supervision. \Charlie{not sure if I should cite latent-nerf}

% \paragraph{Multimodal 3D Generation}
% Dream Fields~\cite{Jain:2022DreamFields}, TextCraft~\cite{Sanghi:2022Textcraft}, and CLIP-Forge~\cite{Sanghi:2022ClipForge} generate 3D through a differential rendering scheme with CLIP~\cite{Radford:2021CLIP} as guidance.
% ShapeCrafter~\cite{Fu:2022Shapecrafter} recursively generate new shape based on previous shape and portion of the prompt.
% AutoSDF~\cite{Mittal:2022Autosdf} and Text2Shape~\cite{Chen:2018Text2shape} learn shape embeddings for 3D generation.

% \paragraph{Diffusion Probabilistic Models}
% Diffusion probabilistic model (DDPM)~\cite{Ho:2019DDPM} is one class of the latent variable models. Compared to other generative models, variational autoencoder (VAE)~\cite{Kingma:2014VAE}, generative adversarial networks (GAN)~\cite{Goodfellow:2014GAN} and flow-based generative models~\cite{flow}, it has shown state-of-the-art performance in modeling a data distribution of 2D images~\cite{Ho:2019DDPM, Dhariwal:2021DiffusionBeatGANs, Rombach:2022LDM}. Rombach~\etal~\cite{Rombach:2022LDM} has proposed a latent diffusion model

% \paragraph{3D Shape Representation.}
% Local Deep Implicit Functions (LDIF)~\cite{Genova:2020LDIF}. 
% Hao~\etal~\cite{Hao:2020Dualsdf} proposes a joint latent of a fine-grained detail shape and its primitive-based coarse proxy shape where the shape can be manipulated by moving primitives.
% Hui~\etal~\cite{Hui:2022NeuralTemplate} proposes two disentangled shape latent codes, one determines the topolgy of a shape and the other refines the rough template shape.
% SPAGHETTI~\cite{Hertz:2022Spaghetti} proposes to learn disentangled representations for 3D, and allows for sampling from the learned shape prior distribution. The disentangled part representation allow user to deform the final shape by apply affine transformations on the corresponding Gaussian primitives.  


==> iccv2023AuthorKit/old/4_Method_old.tex <==
\section{SALAD - Part-Level Cascaded Diffusion}
\label{sec:method}
% \begin{figure*}[t!]
%     \centering
%     \dummyfig{0.98\linewidth}{0.4\linewidth}{Overall pipeline of our cascaded diffusion model with a conditional encoder and a decoder.}
%     \caption{An overview of our two-stage cascaded latent diffusion model. The first stage latent diffusion model learns a distribution of extrinsic latents. The second stage latent diffusion model learns a conditional distribution of intrinsic latents given extrinsics.}
%     \label{fig:our_pipeline}
% \end{figure*}


% To design a compact 3D shape generative model that can produce high-quality shapes while also being capable of manipulating shapes in a part level, we propose a part-level latent diffusion model. 
% on part-level of shapes, we utilize a object representation proposed by Hertz~\etal~\cite{Hertz:2022Spaghetti}. 

\Charlie{This paragraph briefly summarize the entire section}
To design a diffusion model that could leverage the part-based representation, we first propose a single phase diffusion model that directly learn the distribution of part latents. However, as demonstrated in \ref{sec:experiment}, this model lack the capability to \Charlie{output high quality generation or diversity depends on experiment result}. Motivated by recent work in diffusion models by Ho~\etal~\cite{Ho:2022CascadedLDM}, we propose a cascaded diffusion model design that independently learn the distribution of extrinsic and intrinsic representation. Finally, we show that the later design could be further extended for fine-grained conditional generation which the single phase model could not.

%%%%


%%%%

 \subsection{Single Phase Diffusion Model}
Following Rombach~\etal~\cite{Rombach:2022LDM}, we are interested in modeling distribution of latents. Specifically, in this work, we model the distribution of a set of part latents. 
% Let $\B{P} \in \Real^{N\times D}$ be a set of $\B{p}_i$ encapsulating the information of a 3D shape. 
Let $\{\B{p}_i\} \in \Real^{N\times D}$ be a set of $\B{p}_i$ encapsulating the information of a 3D shape.
As discussed in Sec.~\ref{sec:background_ddpm}, a diffusion model is trained to predict gaussian noise $\Veps$ added to $\{\B{p}_i\}$ at every timestep $t$: 
\begin{equation}
\begin{aligned}
\label{eq:simple_loss}
    \mathcal{L}_{\text{simple}} := \mathbb{E}_{t,\{\B{p}_i\},\Veps\sim \mathcal{N}(0, \B{I})} [ \Vert \Veps - \Veps_{\theta}(\{\B{p}_i^{(t)}\},\gamma(t)) \Vert_2^2],
\end{aligned}
\end{equation}
where $\{\B{p}_i^{(t)}\}$ is noisy set of part latents at timestep $t$, and $\gamma(\cdot)$ is a positional encoding that maps $\Real$ to a higher-dimensional space $\Real^{L}$.~\Juil{equation of positional encoding?} Unlike 2D images, our representation is irregular and forms a set that is permutation invariant. Thus, inspired by Lee~\etal~\cite{Lee:2019SetTF}, we implement a network by Transformer~\cite{Vaswani:2017Attention} instead of U-Net~\cite{Unet} which is a \emph{de facto} standard architecture of 2D diffusion models. Except for essential modifications for conditioning, mainly timestep $t$, we faithfully follow standard Transformer encoder architecture which consists of a stack of self-attention layers and fully-connected layers. When we take into account of conditions to the network, we insert an adaptive layer normalization (adaLN)~\cite{adaln} operation after each fully-connected layer, following the widespread usage in GANs~\cite{Karras:2020StyleGAN2} and diffusion models~\cite{Ho:2019DDPM, Luo:2021DPM}. 

In short, Figure~\ref{fig:transformer_block} depicts an overview of our single-phase model. The network takes the embeddings of input latents, and timestep $t$ scales and shifts every intermediate feature through the adaLN operation. Finally, the time-conditioned Transformer encoder predicts noise through self-attention layers. However, this na\"ive latent diffusion model fails to produce high fidelity shapes. Thus, we propose a cascaded latent diffusion model.

\subsection{Cascaded Latent Diffusion Model}
In this section, we describe our cascaded latent diffusion model. As discussed in Sec.~\ref{sec:background_part_representation}, our part-level representation $\B{p}_i$ is further separated into $\B{e}_i$ and $\B{s}_i$ which entail an input shape's overall rough structure, and fine-detailed surface information, respectively. We observe that it is much easier to first build rough geometry and then fill in the remaining details than to capture all the information of a shape at once, as similar as an artist who frames a sketch and then adds details. From this perspective, to fully leverage the advantage of this representation, we design a two-phase training strategy, inspired by Ho~\etal~\cite{Ho:2022CascadedLDM}. The first phase mdoel parameterized by $\phi$ is an unconditional latent diffusion model which predicts noise on $\{\B{e}_i\}\in\Real^{N\times D_e}$. 

We found that extrinsic parameters contain elements with unstable numerical values such as $\pi$ and $\boldsymbol{\lambda}$. After normalizing these elements based on element-wise means $\mu_i$ and standard deviations $\sigma_i$ of all training data following \ref{eq:normalizing}, our model perform significantly better. 

\begin{equation}
    \hat{x}_i = \cfrac{(x_i - \mu_i)}{\sigma_i}.
\label{eq:normalizing}
\end{equation}
This result agrees with previous work of Rombach~\etal~\cite{Rombach:2022LDM} on how avoiding arbitrary high-variance latent space during training could lead to better network performance. At inference time, we rescale these elements by the means and standard deviations.

% As Rombach~\etal~\cite{Rombach:2022LDM} stated, to avoid arbitrary high-variance latent space during training of the latent diffusion model, we normalize these elements based on element-wise means $\mu_i$ and standard deviations $\sigma_i$ of all training data.
% \begin{equation}
%     \hat{x}_i = \sigma_i x_i + \mu_i
% \end{equation}

On the other hand, the second phase model parameterized by $\psi$ is a \emph{conditional} latent diffusion model. It models a conditional distribution $p(\{\B{s}_i\} \vert \{\B{e}_i\})$ which leverages $\{\B{e}_i\}$ . 
The second phase model is implemented by consecutive two Transformer encoders. The first encoder encodes $\B{e}_i$ to global-aware extrinsic embeddings $f(\B{e}_i)$. The following Transformer encoder is conditioned by a concatenation of $f(\B{e}_i)$ and $\gamma(t)$. Since the correspondence between $\B{e}_i$ and $\B{s}_i$ is given in training, we do not apply cross-attention between them. 

In summary, the training objective function for each phase is summarized by:
\begin{align}
    \mathcal{L}_{ext} &= \mathbb{E}_{t,\{\B{e}_i\},\Veps} [ \Vert \Veps - \Veps_{\phi}(\{\B{e}^{(t)}_i\}, \gamma(t)) \Vert_2^2], \\
    \mathcal{L}_{int} &= \mathbb{E}_{t,\{\B{e}_i\},\{\B{s}_i\},\Veps} [ \Vert \Veps - \Veps_{\psi}(\{\B{s}^{(t)}_i\}, \gamma(t) |\,\{\B{e}_i\}) \Vert_2^2].
\end{align}

To generate a 3D shape at inference time, we sample the latents sequentially. First, we sample extrinsic set $\{\hat{\B{e}}_i\}$ from the first phase model, followed by the rescaling of the elements which are normalized in training. To obtain the correspoinding intrinsic latents set $\{\hat{\B{s}}_i\}$, we feed $\{\hat{\B{e}}_i\}$ into the second phase model. Finally, by feeding the sampled $\{ \hat{\B{e}}_i \}$ and $\{ \hat{\B{s}}_i \}$ to the pre-trained decoder $\mathcal{D}$, we can obtain the neural implicit representation of a generated shape according to Equation~\ref{eq:decoder}.
% \begin{equation}
%     \mathcal{L}_{ext} = \cfrac{1}{M} \sum_{j}^{M} \mathbb{E}_{\Ve_j ,t, \Veps \sim \mathcal{N}(0,\mathbf{I})} || \Veps - \Veps_\theta( \Ve_j^{(t)}, \gamma(t))||_2^2,
% \label{eq:phase1_loss}
% \end{equation}



% The phase one model is an unconditional latent diffusion model~\cite{Rombach:2022LDM} with $\{\Ve_j\}$. 
% where $\Ve_j^{(t)}$ indicates a noised\Charlie{noisy} extrinsic latent at timestep $t$ and $\gamma(\cdot)$ is a positional encoding. The phase 1 model $\Veps_\theta$ is implemented as a variant of the Transformer encoder: a stack of self-attention layers and MLPs. 

% By predicting noises at every uniformly sampled timestep $t$ as Equation~\ref{eq:phase1_loss}, the model learns the distribution of extrinsic latents. \Juil{We might need to include index encoding.}
% % As Rombach~\etal~\cite{Rombach:2022LDM} stated that it is crucial to avoid arbitrary high-variance latent space during training of the diffusion model, we normalize elements with unstable numerical values, $\pi$ and $\boldsymbol{\lambda}$, by element-wise means $\mu_i$ and standard deviations $\sigma_i$ pre-computed from all training data. In inference time, we re-scale these elements:
% However, we found that ground truth latents contain elements with unstable numerical values such as $\pi$ and $\boldsymbol{\lambda}$. After normalizing these elements based on element-wise means $\mu_i$ and standard deviations $\sigma_i$ of all training data following \ref{eq:normalizing}, our model perform significantly better. 
% \begin{equation}
%     \hat{x}_i = \sigma_i x_i + \mu_i.
% \label{eq:normalizing}
% \end{equation}
% This result agree with previous work of Rombach~\etal~\cite{Rombach:2022LDM} on how avoiding arbitrary high-variance latent space during training could lead to better network performance.

% Our phase two model is a \emph{conditional} latent diffusion model which models a conditional distribution $p(\Vs_j | \Ve_j)$. 
% \begin{equation}
%     \mathcal{L}_{int} = \cfrac{1}{M} \sum_{j}^{M} \mathbb{E}_{ \Ve_j,\Vs_j,t,\Veps\sim \mathcal{N}(0,\mathbf{I})} || \Veps - \Veps_\phi (\Vs_j^{(t)}, \gamma(t) |\, \Ve_j) ||_2^2
% \end{equation}
% Given a noised \Charlie{noisy} intrinsic latent $\Vs_j^{(t)}$ at time step $t$ and $\Ve_j$ as a condition, the phase 2 model $\Veps_\phi$ predicts noises $\Veps$. To condition both $\gamma(t)$ and $\Ve_j$ on the phase 2 model, we concatenate $\gamma(t)$ and embeddings of $\Ve_j$ as condition. The phase 2 model is implemented by two Transformer encoders where the first encoder embeds $\Ve_j$ to $h(\Ve_j)$ and the other encoder replace MLPs with TMLPs conditioned by $\gamma(t)$ and $h(\Ve_j)$. 

% To generate a 3D shape in test time, we first sample $\{\hat{\Ve}_j\}$ from the phase 1 model and feed them to the phase 2 model to obtain the corresponding $\{\hat{\Vs}_j\}$. Lastly, the pre-trained decoder $\mathcal{D}$ returns an implicit field from the sampled $\{\hat{\Ve}_j\}$ and $\{\hat{\Vs}_j\}$.

% \subsection{Conditioning Mechanism}
% Our network is agnostic to arbitrary additional conditions. When additional condition $c$ is given, we can extract 

==> tables/shape_generation_more_results.tex <==
\begin{table*}[h!]
\centering
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\caption{\textbf{More quantitative comparisons of shape generation.} We report the means and standard deviations of Neural Wavelet and \salad{} results based on \emph{five} random samplings. MMD-CD scores and MMD-EMD scores are scaled by $10^3$ and $10^2$, respectively.}
\footnotesize
{
\setlength{\tabcolsep}{0.2em}
\renewcommand{\arraystretch}{1.0}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.85}
\begin{tabularx}{\linewidth}{>{\centering}m{3.0cm}| Y Y Y Y Y Y | Y Y Y Y Y Y }
  \toprule
  \multirow{3}{*}{Method} & \multicolumn{6}{c|}{Chair} & \multicolumn{6}{c}{Airplane} \\
                 & \multicolumn{2}{c}{COV $\uparrow$} & \multicolumn{2}{c}{MMD $\downarrow$} & \multicolumn{2}{c|}{1-NNA $\downarrow$}  & \multicolumn{2}{c}{COV $\uparrow$} & \multicolumn{2}{c}{MMD $\downarrow$} & \multicolumn{2}{c}{1-NNA $\downarrow$} \\
                         &   CD   &   EMD   &   CD   &   EMD   &   CD   &   EMD   &   CD   &   EMD   &   CD   &   EMD   &   CD   &   EMD \\
  \midrule
  % Diff. of $\{(\B{e}_i, \B{s}_i)\}_{i=1}^N$ & 52.36 &	\textbf{55.01} &	14.56 &	15.86 &	66.92 &	64.31 & 54.02 &	62.05 &	4.551 &	9.627 &	82.76 &	78.99 \\
  Neural Wavelet~\cite{Hui:2022NeuralWavelet}   & \makecell{49.84 \\ $\pm$ 0.96} & \makecell{50.35 \\ $\pm$ 0.95} & \makecell{12.02 \\ $\pm$ 0.08} & \makecell{\textbf{14.23} \\ $\pm$ 0.04} & \makecell{64.12 \\ $\pm$ 0.95} & \makecell{62.71 \\ $\pm$ 0.44} & \makecell{61.16 \\ $\pm$ 0.60} & \makecell{60.94 \\ $\pm$ 1.09} & \makecell{3.552 \\ $\pm$ 0.079} & \makecell{7.979 \\ $\pm$ 0.049} & \makecell{72.64 \\ $\pm$ 2.19} & \makecell{70.83 \\ $\pm$ 1.66} \\
  
  \midrule 
\salad{} (Ours)                  & \makecell{\textbf{55.46}\\$\pm$1.30} & \makecell{54.84\\$\pm$0.56} &	\makecell{\textbf{11.84}\\$\pm$0.11} & \makecell{14.32\\$\pm$0.03} &	\makecell{\textbf{58.42}\\$\pm$1.09} &	\makecell{\textbf{58.17}\\$\pm$1.30} &	\makecell{62.50\\$\pm$1.30} &	\makecell{64.23\\$\pm$0.68} & \makecell{3.621\\$\pm$0.022} & \makecell{8.283\\$\pm$0.028} &	\makecell{74.13\\$\pm$0.99} & \makecell{71.58\\$\pm$0.56} \\
  \bottomrule
\end{tabularx}
}
\vspace{-0.5\baselineskip}
\label{tbl:more_quantitative_comparison_of_shape_generation}
\end{table*}

